M-RAG: Reinforcing Large Language Model Performance through Retrieval-Augmented Generation with Multiple Partitions

Retrieval-Augmented Generation (RAG) enhances Large Language Models (LLMs) by retrieving relevant memories from an external database. However, existing RAG methods typically organize all memories in a whole database, potentially limiting focus on crucial memories and introducing noise. In this paper, we introduce a multiple partition paradigm for RAG (called M-RAG), where each database partition serves as a basic unit for RAG execution. Based on this paradigm, we propose a novel framework that leverages LLMs with Multi-Agent Reinforcement Learning to optimize different language generation tasks explicitly. Through comprehensive experiments conducted on seven datasets, spanning three language generation tasks and involving three distinct language model architectures, we confirm that M-RAG consistently outperforms various baseline methods, achieving improvements of 11%, 8%, and 12% for text summarization, machine translation, and dialogue generation, respectively.

==> experiment.tex <==
\subsection{Experimental Results}
\label{sec:result}

\begin{figure*}[ht]
	\centering
	\hspace*{-4mm}
	\begin{tabular}{c c c c}
 	\hspace{-3mm}
		\begin{minipage}{0.25\textwidth}%5.5
			\includegraphics[width=\textwidth]{figures/summarization.pdf}
		\end{minipage}\hspace{-3mm}
		&
		\begin{minipage}{0.25\textwidth}
			\includegraphics[width=\textwidth]{figures/summarization_topK_time.pdf}
		\end{minipage}\hspace{-3mm}
		&
		\begin{minipage}{0.25\textwidth}
			\includegraphics[width=\textwidth]{figures/translation_esen.pdf}
		\end{minipage}\hspace{-3mm}
		&
		\begin{minipage}{0.25\textwidth}
			\includegraphics[width=\textwidth]{figures/dialogue.pdf}
		\end{minipage}\hspace{-3mm}
		\\
		(a) Summ. (ROUGE-1) 
		&
		(b) Summ. (Runtime) 
		&
		(c) Machine translation
		&
		(d) Dialogue generation

	\end{tabular}
 	\vspace*{-3mm}
	\caption{Comparison with database partitioning strategies for language generation tasks.}\label{fig:partition}
	\vspace*{-1mm}
\end{figure*}

\begin{table*}[t]
\caption{Text summarization.}
\centering
\vspace{-3mm}
\label{tab:summarization}
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|c|c|ccc|ccc}
\hline
\multicolumn{2}{l|}{\multirow{2}{*}{LLM}}  & \multirow{2}{*}{RAG} & \multicolumn{3}{c|}{XSum} & \multicolumn{3}{c}{BigPatent} \\ \cline{4-9} 
\multicolumn{2}{l|}{}                      &                      & R-1     & R-2    & R-L    & R-1      & R-2      & R-L     \\ \hline
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & None                &    25.40      &   6.39     &   18.30     &          &          &         \\
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & Naive              & 43.82 & 22.07 & 37.44        &          &          &         \\
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & Selfmem              &   39.67      &  14.38     &   31.86     &          &          &         \\
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & Self-RAG             &    33.01     &  12.56      &    27.51    &          &          &         \\ \hline
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & \texttt{M-RAG}                & \textbf{48.13}    & \textbf{24.66}  & \textbf{39.43}        &          &          &         \\
\multicolumn{2}{l|}{Llama 2 13B}           & \texttt{M-RAG}               &    37.18     &   18.02     &    26.44    &          &          &         \\
\multicolumn{2}{l|}{Phi-2 2.7B}            & \texttt{M-RAG}                &    30.70     &  11.57      &    26.20    &     31.25     &    8.72      &    18.98     \\ \hline
\end{tabular}
\end{table*}

\noindent \textbf{(1) Effectiveness evaluation (partitioning strategies).} We conduct experiments to evaluate various partitioning strategies across text summarization (XSum), machine translation (Es$\rightarrow$En), and dialogue generation (DailyDialog) tasks with Mixtral 8 $\times$ 7B. The best results, based on a development set across different partitions, are reported. As shown in Figure~\ref{fig:partition}, we observe that retrieval based on the entire database generally fails to achieve optimal performance. Moreover, the performance slightly decreases as the number of partitions increases. This is attributed to the AKNN search, where a smaller partition size recalls more similar memories, which may not align well with the LLM preferences and impede the focus on crucial memories. Additionally, we observe that the RAG with Top-1 retrieval exhibits faster runtime compared to the Top-3 due to a shorter input length for the LLM, while maintaining comparable performance.

\begin{table*}[t]
\caption{Machine translation.}
\centering
\vspace{-3mm}
\label{tab:translation}
\begin{tabular}{l|c|c|cc|cc|cc|cc}
\hline
\multicolumn{2}{l|}{\multirow{2}{*}{LLM}} & \multirow{2}{*}{RAG} & \multicolumn{2}{c|}{Es$\rightarrow$En} & \multicolumn{2}{c|}{En$\rightarrow$Es} & \multicolumn{2}{c|}{De$\rightarrow$En} & \multicolumn{2}{c}{En$\rightarrow$De} \\ \cline{4-11} 
\multicolumn{2}{l|}{}                     &                      & Dev               & Test               & Dev               & Test               & Dev               & Test               & Dev               & Test              \\ \hline
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & None                 &         42.64          &          24.81          &            22.60       &          19.32         &             39.75      &         27.77           &              35.78     &       21.24           \\
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & Naive              &        38.34           &         26.22            &        35.18           &          32.70          &            47.84       &         19.09           &               45.83    &        48.23           \\
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & Selfmem              &                   &                    &                   &                    &                   &                    &                   &                   \\
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & Self-RAG             &         38.17          &           28.82         &         12.80          &         9.61           &            22.69       &         11.27           &   2.10                &         5.75          \\ \hline
\multicolumn{2}{l|}{Mixtral 8 $\times$ 7B} & \texttt{M-RAG}                &         39.11          &    29.98                &       35.18            &      32.70              &       49.16            &      44.15              &       53.76            &      46.75            \\
\multicolumn{2}{l|}{Llama 2 13B}          & \texttt{M-RAG}                &      30.41             &      18.03              &        19.40           &       12.03             &      24.10             &        22.22            &       31.98            &        31.58           \\
\multicolumn{2}{l|}{Phi-2 2.7B}           & \texttt{M-RAG}                &    20.83               &       4.22             &       17.64            &          6.60          &         4.21          &          0.71          &      10.01             &        1.08           \\ \hline
\end{tabular}
\end{table*}


\begin{table}[t]
\caption{Dialogue generation.}
\setlength{\tabcolsep}{1.8pt}
\vspace{-3mm}
\label{tab:dialogue}
\begin{tabular}{l|c|c|cccc}
\hline
\multicolumn{2}{l|}{\multirow{2}{*}{LLM}}  & \multirow{2}{*}{RAG} & \multicolumn{4}{c}{DailyDialog} \\ \cline{4-7} 
\multicolumn{2}{l|}{}                      &                      & B-1    & B-2    & D-1   & D-2   \\ \hline
\multicolumn{2}{l|}{Mix. 8 $\times$ 7B} & None                 &        &        &       &       \\
\multicolumn{2}{l|}{Mix. 8 $\times$ 7B} & Naive              &        &        &       &       \\
\multicolumn{2}{l|}{Mix. 8 $\times$ 7B} & Selfmem              &        &        &       &       \\
\multicolumn{2}{l|}{Mix. 8 $\times$ 7B} & Self-RAG             &        &        &       &       \\ \hline
\multicolumn{2}{l|}{Mix. 8 $\times$ 7B} & \texttt{M-RAG}             &        &        &       &       \\
\multicolumn{2}{l|}{Llama 2 13B}           & \texttt{M-RAG}                &        &        &       &       \\
\multicolumn{2}{l|}{Phi-2 2.7B}            & \texttt{M-RAG}                &        &        &       &       \\ \hline
\multicolumn{2}{l|}{Mix. 8 $\times$ 7B} & \texttt{M-RAG} (D)                &        &        &       &  \\ \hline
\end{tabular}
\end{table}

\noindent \textbf{(2) Effectiveness evaluation (text summarization).} 
We compare the performance of the \texttt{M-RAG} against alternative RAG methods on three distinct language models: Mixtral 8$\times$7B, Llama 2 13B, and Phi-2 2.7B. The corresponding results are outlined in Table~\ref{tab:summarization}.


\noindent \textbf{(3) Effectiveness evaluation (machine translation).} 
We further conduct experiments to evaluate the performance of \texttt{M-RAG} for machine translation, and the results are reported in Table~\ref{tab:translation}.

\noindent \textbf{(4) Effectiveness evaluation (dialogue generation).}
As shown in Table~\ref{tab:dialogue}, \texttt{M-RAG} further enhances the language model performance for dialogue generation tasks. 

\begin{table}[t]
\caption{Ablation study.}
\setlength{\tabcolsep}{4pt}
\vspace{-3mm}
\label{tab:ablation}
\begin{tabular}{cccc}
\hline
Components                 & R-1 & R-2 & R-L \\ \hline
\texttt{M-RAG}                    & \textbf{48.13}    & \textbf{24.66}  & \textbf{39.43} \\ \hline
w/o Agent-S (single DB) & 44.20 & 22.72 &  37.40  \\
w/o Agent-R (greedy)      & 45.75 & 23.21 & 38.28   \\ \hline
w/o Agent-S and Agent-R       & 43.82 & 22.07 & 37.44   \\ \hline
\end{tabular}
%\vspace*{-3mm}
\end{table}


\noindent \textbf{(5) Ablation study.} To evaluate the effectiveness of the two agents in \texttt{M-RAG}, we conduct an ablation study on XSum. We remove Agent-S and utilize the entire database for RAG; we replace Agent-R with a greedy rule to select a candidate memory from the pool according to Equation~\ref{eq:state_r}; and we remove both agents, which degrades to the Naive RAG. The results are presented in Table~\ref{tab:ablation}, demonstrating that both agents contribute to performance improvement. Specifically, removing Agent-S results in a significant decline in R-1 from 48.13 to 44.20. This underscores the role of the multiple partition setting in enhancing overall performance. Moreover, removing Agent-R leads to a reduction in R-1 from 48.13 to 45.75. This decline is attributed to the effectiveness of Agent-R in learning memory selection dynamically, as opposed to relying on a fixed rule for decision-making.

\begin{table}[t]
\setlength{\tabcolsep}{2.2pt}
\caption{Impacts of the number of $M$ in Agent-S.}
\vspace{-3mm}
\label{tab:parameter_m}
\begin{tabular}{c|ccccc}
\hline
$M$ & 1 & 2 & 3 & 4 & 5 \\ \hline
R-1       &44.20 & & &48.13 &    \\
Index constr. (s) & 299 & 327 & 327 & 329 & 327   \\
Retrieval (s)      & 0.61 & 1.95 & 2.15 & 2.19 & 2.79\\
Generation (s)     & 83.59 & 84.88 & 72.81 & 82.89 & 76.64 \\
%ROUGE-2       & & & & &     \\
%ROUGE-L  & & & & &     \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[t]
\setlength{\tabcolsep}{3.4pt}
\caption{Impacts of the number of $K$ in Agent-R.}
\vspace{-3mm}
\label{tab:parameter_k}
\begin{tabular}{c|ccccc}
\hline
$K$ & 1 & 2 & 3 & 4 & 5 \\ \hline
R-1       & & & 48.13 & &    \\
Pool gen. (s)       & 76.53 & 79.43 & 82.03 & 78.43 & 81.12   \\
% Time (s)       & & & & &     \\
% ROUGE-2       & & & & &     \\
% ROUGE-L  & & & & &     \\ 
\hline
\end{tabular}
\end{table}

\noindent \textbf{(6) Parameter study (Agent-S state space $M$).} We study the effect of parameter $M$, which controls
the state space of Agent-S and corresponds to the number of partitions. {\Zheng In Table~\ref{tab:parameter_m}, we observe that setting $M = xx$ yields the best effectiveness while maintaining reasonable runtime in terms of index construction, retrieval, and generation. This is consistent with empirical studies illustrated in Figure~\ref{fig:partition} (a). When $M=1$, it reduces to a single database for RAG. As $M$ increases, index construction accelerates on smaller partitions, while retrieval time remains stable due to the additional time required for constructing states by querying each partition. As expected, the retrieval time is much smaller than the language generation time.
}

\noindent \textbf{(7) Parameter study (Agent-R state space $K$).} We study the effect of parameter $K$ in Agent-R, representing the state space of Agent-R, to choose one memory from a candidate pool with a size of $K$. {\Zheng In Table~\ref{tab:parameter_k}, we observe a performance improvement as $K$ increases from xx to xx, followed by a decline when $K$ becomes xx. Particularly, when $K=1$, \texttt{M-RAG} exhibits the worst performance, possibly due to the limited exploration of potential memories for generating improved hypotheses. We choose the setting of $K=xx$, as it demonstrates the best effectiveness.
}


